Canonical Supermartingale Couplings

Two probability distributions $\mu$ and $\nu$ in second stochastic order can be coupled by a supermartingale, and in fact by many. Is there a canonical choice? We construct and investigate two couplings which arise as optimizers for constrained Monge-Kantorovich optimal transport problems where only supermartingales are allowed as transports. Much like the Hoeffding-Fr\'echet coupling of classical transport and its symmetric counterpart, the antitone coupling, these can be characterized by order-theoretic minimality properties, as simultaneous optimal transports for certain classes of reward (or cost) functions, and through no-crossing conditions on their supports; however, our two couplings have asymmetric geometries. Remarkably, supermartingale optimal transport decomposes into classical and martingale transport in several ways.

==> simulationIncr_pic.tex <==
\resizebox{4.2in}{!}{
\begin{tikzpicture}[every node/.style={draw,circle,fill=black,inner sep=0pt,minimum size=0.5pt}]

\draw[thick] (-6,0) -- (10,0);\draw[thick] (-6,-3) -- (10,-3);
\node (x0) at (6.0,0) {};
\node (x2) at (6.06,0) {};
\node (x4) at (6.12,0) {};
\node (x6) at (6.18,0) {};
\node (x8) at (6.24,0) {};
\node (x10) at (6.3,0) {};
\node (x12) at (6.36,0) {};
\node (x14) at (6.42,0) {};
\node (x16) at (6.48,0) {};
\node (x18) at (6.54,0) {};
\node (x20) at (6.6,0) {};
\node (x22) at (6.66,0) {};
\node (x24) at (6.72,0) {};
\node (x26) at (6.78,0) {};
\node (x28) at (6.84,0) {};
\node (x30) at (6.9,0) {};
\node (x32) at (6.96,0) {};
\node (x34) at (7.02,0) {};
\node (x36) at (7.08,0) {};
\node (x38) at (7.14,0) {};
\node (x40) at (7.2,0) {};
\node (x42) at (7.26,0) {};
\node (x44) at (7.32,0) {};
\node (x46) at (7.38,0) {};
\node (x48) at (7.44,0) {};
\node (x50) at (7.5,0) {};
\node (x52) at (7.56,0) {};
\node (x54) at (7.62,0) {};
\node (x56) at (7.68,0) {};
\node (x58) at (7.74,0) {};
\node (x60) at (7.8,0) {};
\node (x62) at (7.86,0) {};
\node (x64) at (7.92,0) {};
\node (x66) at (7.98,0) {};
\node (x68) at (8.04,0) {};
\node (x70) at (8.1,0) {};
\node (x72) at (8.16,0) {};
\node (x74) at (8.22,0) {};
\node (x76) at (8.28,0) {};
\node (x78) at (8.34,0) {};
\node (x80) at (8.4,0) {};
\node (x82) at (8.46,0) {};
\node (x84) at (8.52,0) {};
\node (x86) at (8.58,0) {};
\node (x88) at (8.64,0) {};
\node (x90) at (8.7,0) {};
\node (x92) at (8.76,0) {};
\node (x94) at (8.82,0) {};
\node (x96) at (8.88,0) {};
\node (x98) at (8.94,0) {};
\node (x100) at (9.0,0) {};
\node (y0) at (-4.5,-3) {};
\node (y2) at (-4.44,-3) {};
\node (y4) at (-4.38,-3) {};
\node (y6) at (-4.32,-3) {};
\node (y8) at (-4.26,-3) {};
\node (y10) at (-4.2,-3) {};
\node (y12) at (-4.14,-3) {};
\node (y14) at (-4.08,-3) {};
\node (y16) at (-4.02,-3) {};
\node (y18) at (-3.96,-3) {};
\node (y20) at (-3.9,-3) {};
\node (y22) at (-3.84,-3) {};
\node (y24) at (-3.78,-3) {};
\node (y26) at (-3.72,-3) {};
\node (y28) at (-3.66,-3) {};
\node (y30) at (-3.6,-3) {};
\node (y32) at (-3.54,-3) {};
\node (y34) at (-3.48,-3) {};
\node (y36) at (-3.42,-3) {};
\node (y38) at (-3.36,-3) {};
\node (y40) at (-3.3,-3) {};
\node (y42) at (-3.24,-3) {};
\node (y44) at (-3.18,-3) {};
\node (y46) at (-3.12,-3) {};
\node (y48) at (-3.06,-3) {};
\node (y50) at (-3.0,-3) {};
\node (y52) at (3.03,-3) {};
\node (y54) at (3.09,-3) {};
\node (y56) at (3.15,-3) {};
\node (y58) at (3.21,-3) {};
\node (y60) at (3.27,-3) {};
\node (y62) at (3.33,-3) {};
\node (y64) at (3.39,-3) {};
\node (y66) at (3.45,-3) {};
\node (y68) at (3.51,-3) {};
\node (y70) at (3.57,-3) {};
\node (y72) at (3.63,-3) {};
\node (y74) at (3.69,-3) {};
\node (y76) at (3.75,-3) {};
\node (y78) at (3.81,-3) {};
\node (y80) at (3.87,-3) {};
\node (y82) at (3.93,-3) {};
\node (y84) at (3.99,-3) {};
\node (y86) at (4.05,-3) {};
\node (y88) at (4.11,-3) {};
\node (y90) at (4.17,-3) {};
\node (y92) at (4.23,-3) {};
\node (y94) at (4.29,-3) {};
\node (y96) at (4.35,-3) {};
\node (y98) at (4.41,-3) {};
\node (y100) at (4.47,-3) {};
\draw[color=gray] (x0) -- (y100);
\draw[color=gray] (x2) -- (y98);
\draw[color=gray] (x4) -- (y96);
\draw[color=gray] (x6) -- (y94);
\draw[color=gray] (x8) -- (y92);
\draw[color=gray] (x10) -- (y90);
\draw[color=gray] (x12) -- (y88);
\draw[color=gray] (x14) -- (y86);
\draw[color=gray] (x16) -- (y84);
\draw[color=gray] (x18) -- (y82);
\draw[color=gray] (x20) -- (y80);
\draw[color=gray] (x22) -- (y78);
\draw[color=gray] (x24) -- (y76);
\draw[color=gray] (x26) -- (y74);
\draw[color=gray] (x28) -- (y72);
\draw[color=gray] (x30) -- (y70);
\draw[color=gray] (x32) -- (y68);
\draw[color=gray] (x34) -- (y66);
\draw[color=gray] (x36) -- (y64);
\draw[color=gray] (x38) -- (y62);
\draw[color=gray] (x40) -- (y60);
\draw[color=gray] (x42) -- (y58);
\draw[color=gray] (x44) -- (y56);
\draw[color=gray] (x46) -- (y54);
\draw[color=gray] (x48) -- (y52);
\draw[color=gray] (x50) -- (y50);
\draw[color=gray] (x52) -- (y48);
\draw[color=gray] (x54) -- (y46);
\draw[color=gray] (x56) -- (y44);
\draw[color=gray] (x58) -- (y42);
\draw[color=gray] (x60) -- (y40);
\draw[color=gray] (x62) -- (y38);
\draw[color=gray] (x64) -- (y36);
\draw[color=gray] (x66) -- (y34);
\draw[color=gray] (x68) -- (y32);
\draw[color=gray] (x70) -- (y30);
\draw[color=gray] (x72) -- (y28);
\draw[color=gray] (x74) -- (y26);
\draw[color=gray] (x76) -- (y24);
\draw[color=gray] (x78) -- (y22);
\draw[color=gray] (x80) -- (y20);
\draw[color=gray] (x82) -- (y18);
\draw[color=gray] (x84) -- (y16);
\draw[color=gray] (x86) -- (y14);
\draw[color=gray] (x88) -- (y12);
\draw[color=gray] (x90) -- (y10);
\draw[color=gray] (x92) -- (y8);
\draw[color=gray] (x94) -- (y6);
\draw[color=gray] (x96) -- (y4);
\draw[color=gray] (x98) -- (y2);
\draw[color=gray] (x100) -- (y0);
\node (x300) at (-1.5,0) {};
\node (x302) at (-1.44,0) {};
\node (x304) at (-1.38,0) {};
\node (x306) at (-1.32,0) {};
\node (x308) at (-1.26,0) {};
\node (x310) at (-1.2,0) {};
\node (x312) at (-1.14,0) {};
\node (x314) at (-1.08,0) {};
\node (x316) at (-1.02,0) {};
\node (x318) at (-0.96,0) {};
\node (x320) at (-0.9,0) {};
\node (x322) at (-0.84,0) {};
\node (x324) at (-0.78,0) {};
\node (x326) at (-0.72,0) {};
\node (x328) at (-0.66,0) {};
\node (x330) at (-0.6,0) {};
\node (x332) at (-0.54,0) {};
\node (x334) at (-0.48,0) {};
\node (x336) at (-0.42,0) {};
\node (x338) at (-0.36,0) {};
\node (x340) at (-0.3,0) {};
\node (x342) at (-0.24,0) {};
\node (x344) at (-0.18,0) {};
\node (x346) at (-0.12,0) {};
\node (x348) at (-0.06,0) {};
\node (x350) at (0.0,0) {};
\node (x352) at (0.06,0) {};
\node (x354) at (0.12,0) {};
\node (x356) at (0.18,0) {};
\node (x358) at (0.24,0) {};
\node (x360) at (0.3,0) {};
\node (x362) at (0.36,0) {};
\node (x364) at (0.42,0) {};
\node (x366) at (0.48,0) {};
\node (x368) at (0.54,0) {};
\node (x370) at (0.6,0) {};
\node (x372) at (0.66,0) {};
\node (x374) at (0.72,0) {};
\node (x376) at (0.78,0) {};
\node (x378) at (0.84,0) {};
\node (x380) at (0.9,0) {};
\node (x382) at (0.96,0) {};
\node (x384) at (1.02,0) {};
\node (x386) at (1.08,0) {};
\node (x388) at (1.14,0) {};
\node (x390) at (1.2,0) {};
\node (x392) at (1.26,0) {};
\node (x394) at (1.32,0) {};
\node (x396) at (1.38,0) {};
\node (x398) at (1.44,0) {};
\node (x400) at (1.5,0) {};
\node (y300) at (-3.0,-3) {};
\node (y302) at (-2.94,-3) {};
\node (y304) at (-2.88,-3) {};
\node (y306) at (-2.82,-3) {};
\node (y308) at (-2.76,-3) {};
\node (y310) at (-2.7,-3) {};
\node (y312) at (-2.64,-3) {};
\node (y314) at (-2.58,-3) {};
\node (y316) at (-2.52,-3) {};
\node (y318) at (-2.46,-3) {};
\node (y320) at (-2.4,-3) {};
\node (y322) at (-2.34,-3) {};
\node (y324) at (-2.28,-3) {};
\node (y326) at (-2.22,-3) {};
\node (y328) at (-2.16,-3) {};
\node (y330) at (-2.1,-3) {};
\node (y332) at (-2.04,-3) {};
\node (y334) at (-1.98,-3) {};
\node (y336) at (-1.92,-3) {};
\node (y338) at (-1.86,-3) {};
\node (y340) at (-1.8,-3) {};
\node (y342) at (-1.74,-3) {};
\node (y344) at (-1.68,-3) {};
\node (y346) at (-1.62,-3) {};
\node (y348) at (-1.56,-3) {};
\node (y350) at (-1.5,-3) {};
\node (y352) at (-1.44,-3) {};
\node (y354) at (-1.38,-3) {};
\node (y356) at (-1.32,-3) {};
\node (y358) at (-1.26,-3) {};
\node (y360) at (-1.2,-3) {};
\node (y362) at (-1.14,-3) {};
\node (y364) at (-1.08,-3) {};
\node (y366) at (-1.02,-3) {};
\node (y368) at (-0.96,-3) {};
\node (y370) at (-0.9,-3) {};
\node (y372) at (-0.84,-3) {};
\node (y374) at (-0.78,-3) {};
\node (y376) at (-0.72,-3) {};
\node (y378) at (-0.66,-3) {};
\node (y380) at (-0.6,-3) {};
\node (y382) at (-0.54,-3) {};
\node (y384) at (-0.48,-3) {};
\node (y386) at (-0.42,-3) {};
\node (y388) at (-0.36,-3) {};
\node (y390) at (-0.3,-3) {};
\node (y392) at (-0.24,-3) {};
\node (y394) at (-0.18,-3) {};
\node (y396) at (-0.12,-3) {};
\node (y398) at (-0.06,-3) {};
\node (y400) at (0.0,-3) {};
\node (y402) at (0.06,-3) {};
\node (y404) at (0.12,-3) {};
\node (y406) at (0.18,-3) {};
\node (y408) at (0.24,-3) {};
\node (y410) at (0.3,-3) {};
\node (y412) at (0.36,-3) {};
\node (y414) at (0.42,-3) {};
\node (y416) at (0.48,-3) {};
\node (y418) at (0.54,-3) {};
\node (y420) at (0.6,-3) {};
\node (y422) at (0.66,-3) {};
\node (y424) at (0.72,-3) {};
\node (y426) at (0.78,-3) {};
\node (y428) at (0.84,-3) {};
\node (y430) at (0.9,-3) {};
\node (y432) at (0.96,-3) {};
\node (y434) at (1.02,-3) {};
\node (y436) at (1.08,-3) {};
\node (y438) at (1.14,-3) {};
\node (y440) at (1.2,-3) {};
\node (y442) at (1.26,-3) {};
\node (y444) at (1.32,-3) {};
\node (y446) at (1.38,-3) {};
\node (y448) at (1.44,-3) {};
\node (y450) at (1.5,-3) {};
\node (y452) at (1.56,-3) {};
\node (y454) at (1.62,-3) {};
\node (y456) at (1.68,-3) {};
\node (y458) at (1.74,-3) {};
\node (y460) at (1.8,-3) {};
\node (y462) at (1.86,-3) {};
\node (y464) at (1.92,-3) {};
\node (y466) at (1.98,-3) {};
\node (y468) at (2.04,-3) {};
\node (y470) at (2.1,-3) {};
\node (y472) at (2.16,-3) {};
\node (y474) at (2.22,-3) {};
\node (y476) at (2.28,-3) {};
\node (y478) at (2.34,-3) {};
\node (y480) at (2.4,-3) {};
\node (y482) at (2.46,-3) {};
\node (y484) at (2.52,-3) {};
\node (y486) at (2.58,-3) {};
\node (y488) at (2.64,-3) {};
\node (y490) at (2.7,-3) {};
\node (y492) at (2.76,-3) {};
\node (y494) at (2.82,-3) {};
\node (y496) at (2.88,-3) {};
\node (y498) at (2.94,-3) {};
\node (y500) at (3.0,-3) {};
\draw (x300) -- (y350);
\draw (x302) -- (y348);
\draw (x302) -- (y352);
\draw (x302) -- (y354);
\draw (x304) -- (y348);
\draw (x304) -- (y356);
\draw (x306) -- (y346);
\draw (x306) -- (y358);
\draw (x306) -- (y360);
\draw (x308) -- (y346);
\draw (x308) -- (y362);
\draw (x310) -- (y344);
\draw (x310) -- (y364);
\draw (x310) -- (y366);
\draw (x312) -- (y344);
\draw (x312) -- (y368);
\draw (x314) -- (y342);
\draw (x314) -- (y370);
\draw (x314) -- (y372);
\draw (x316) -- (y342);
\draw (x316) -- (y374);
\draw (x318) -- (y340);
\draw (x318) -- (y376);
\draw (x318) -- (y378);
\draw (x320) -- (y340);
\draw (x320) -- (y380);
\draw (x322) -- (y338);
\draw (x322) -- (y382);
\draw (x322) -- (y384);
\draw (x324) -- (y338);
\draw (x324) -- (y386);
\draw (x326) -- (y336);
\draw (x326) -- (y388);
\draw (x326) -- (y390);
\draw (x328) -- (y336);
\draw (x328) -- (y392);
\draw (x330) -- (y334);
\draw (x330) -- (y394);
\draw (x330) -- (y396);
\draw (x332) -- (y334);
\draw (x332) -- (y398);
\draw (x334) -- (y332);
\draw (x334) -- (y400);
\draw (x334) -- (y402);
\draw (x336) -- (y332);
\draw (x336) -- (y404);
\draw (x338) -- (y330);
\draw (x338) -- (y406);
\draw (x338) -- (y408);
\draw (x340) -- (y330);
\draw (x340) -- (y410);
\draw (x342) -- (y328);
\draw (x342) -- (y412);
\draw (x342) -- (y414);
\draw (x344) -- (y328);
\draw (x344) -- (y416);
\draw (x346) -- (y326);
\draw (x346) -- (y418);
\draw (x346) -- (y420);
\draw (x348) -- (y326);
\draw (x348) -- (y422);
\draw (x350) -- (y324);
\draw (x350) -- (y424);
\draw (x350) -- (y426);
\draw (x352) -- (y324);
\draw (x352) -- (y428);
\draw (x354) -- (y322);
\draw (x354) -- (y430);
\draw (x354) -- (y432);
\draw (x356) -- (y322);
\draw (x356) -- (y434);
\draw (x358) -- (y320);
\draw (x358) -- (y436);
\draw (x358) -- (y438);
\draw (x360) -- (y320);
\draw (x360) -- (y440);
\draw (x362) -- (y318);
\draw (x362) -- (y442);
\draw (x362) -- (y444);
\draw (x364) -- (y318);
\draw (x364) -- (y446);
\draw (x366) -- (y316);
\draw (x366) -- (y448);
\draw (x366) -- (y450);
\draw (x368) -- (y316);
\draw (x368) -- (y452);
\draw (x370) -- (y314);
\draw (x370) -- (y454);
\draw (x370) -- (y456);
\draw (x372) -- (y314);
\draw (x372) -- (y458);
\draw (x374) -- (y312);
\draw (x374) -- (y460);
\draw (x374) -- (y462);
\draw (x376) -- (y312);
\draw (x376) -- (y464);
\draw (x378) -- (y310);
\draw (x378) -- (y466);
\draw (x378) -- (y468);
\draw (x380) -- (y310);
\draw (x380) -- (y470);
\draw (x382) -- (y308);
\draw (x382) -- (y472);
\draw (x382) -- (y474);
\draw (x384) -- (y308);
\draw (x384) -- (y476);
\draw (x386) -- (y306);
\draw (x386) -- (y478);
\draw (x386) -- (y480);
\draw (x388) -- (y306);
\draw (x388) -- (y482);
\draw (x390) -- (y304);
\draw (x390) -- (y484);
\draw (x390) -- (y486);
\draw (x392) -- (y304);
\draw (x392) -- (y488);
\draw (x394) -- (y302);
\draw (x394) -- (y490);
\draw (x394) -- (y492);
\draw (x396) -- (y302);
\draw (x396) -- (y494);
\draw (x398) -- (y300);
\draw (x398) -- (y496);
\draw (x398) -- (y498);
\draw (x400) -- (y300);
\draw (x400) -- (y500);
\end{tikzpicture}}
